Counterfactual Explanations for Face Forgery Detection via Adversarial Removal of Artifacts

Highly realistic AI generated face forgeries known as deepfakes have raised serious social concerns. Although DNN-based face forgery detection models have achieved good performance, they are vulnerable to latest generative methods that have less forgery traces and adversarial attacks. This limitation of generalization and robustness hinders the credibility of detection results and requires more explanations. In this work, we provide counterfactual explanations for face forgery detection from an artifact removal perspective. Specifically, we first invert the forgery images into the StyleGAN latent space, and then adversarially optimize their latent representations with the discrimination supervision from the target detection model. We verify the effectiveness of the proposed explanations from two aspects: (1) Counterfactual Trace Visualization: the enhanced forgery images are useful to reveal artifacts by visually contrasting the original images and two different visualization methods; (2) Transferable Adversarial Attacks: the adversarial forgery images generated by attacking the detection model are able to mislead other detection models, implying the removed artifacts are general. Extensive experiments demonstrate that our method achieves over 90% attack success rate and superior attack transferability. Compared with naive adversarial noise methods, our method adopts both generative and discriminative model priors, and optimize the latent representations in a synthesis-by-analysis way, which forces the search of counterfactual explanations on the natural face manifold. Thus, more general counterfactual traces can be found and better adversarial attack transferability can be achieved.

==> PARTS/related_work.tex <==
\section{Related Work}
\label{sec:related work}

% \subsection{Deepfake Detection}
% Since the dawn of Convolutional Neural Networks (CNNs), Deepfake generation technology has advanced by leaps and bounds in terms of both speed and quality, which causes serious negative social impact. Detection methods~\cite{fingerprinting, proactive, li2021exploring} work on GAN generated person images~\cite{karras2020analyzing, SAN}.  In constrast, we mainly target at a more generalizable Deepfake clues detection models~\cite{cao2022endtoend, zhao2021multi, wang2023altfreezing} despite how the Deepfake images are generated. FTCN~\cite{2021zhengftcn} further takes the temporal conherence into consideration by using a temporal Transformer encoder. Apart from these, F3Net~\cite{qian2020thinking, luo2021generalizing} mine into expose the frequency forgery cues in deepfakes. 

% \subsection{Explanation of Deepfake Detection}
% \label{subsec: explanation of deepfake detection}
% So far, some works use heat-maps to localize the deepfake artifacts use attribution-based methods~\cite{selvaraju2017grad, zhao2023istvt}. Like learning beased fake region location method~\cite{li2020face, guo2023hierarchical}, they only explain where the detector think is fake. And Peng .et al~\cite{peng2022counterfactual} use spatial additive image enhancement techniques to better present subtle artifacts in face swap fake images. However, the only handle with face swap deepfakes which is limited. We propose a method that is deepfake generation process agnostic to show the artifact clues by simply step into changing the facial content to reveal the deepfake clues, with the hypothesis that once the artifact is removed the detectors would consider the new generated face as real. 

\subsection{Adversarial Attacks}
\label{subsec: adversarial attacks}
% Adversarial Examples~\cite{szegedy2013intriguing} are designed to deceive pretrained machine-learning models by adding minor perturbations to the original sample, resulting in an output that differs from the initial one with high confidence. For a classifier $f(\cdot)$ and input $x$, it is possible to construct an additive perturbation $\sigma$ so that $x+\sigma$ is misclassified by $f(\cdot)$. 
For adversarial attacks against general Deepfake detection models. Several existing methods studied the image-level white-box additive perturbation-based attack under different setting~\cite{hussain2021adversarial, neekhara2021adversarial, liao2021imperceptible}. Meanwhile, Jia et al.~\cite{jia2022exploring} launch an attack within the frequency domain to craft more imperceptible adversarial examples. Li et al.~\cite{li2021exploring} optimize the latent code and noise vector to generate fake images of nonexistent person, while ~\cite{xu2021towards} shifts the style distribution to disable the image classifiers. Some previous work~\cite{fakepolisher, liu2023making} have also tried to remove the artifacts in the generated images to evade the supervision of detectors through training a reconstruction decoder. In this paper, we also dive into remove the artifacts left in the Deepfake images. However, we achieve our goal by leveraging the superior prior konwledge of embed in the GAN latent space and using the editing ability of $\mathcal{W}^{18}$ to remove the deepfake tracks.


